Approximation Algorithms for the Two-Watchman Route in a Simple Polygon

The two-watchman route problem is that of computing a pair of closed tours in an environment so that the two tours together see the whole environment and some length measure on the two tours is minimized. Two standard measures are: the minmax measure, where we want the tours where the longest of them has smallest length, and the minsum measure, where we want the tours for which the sum of their lengths is the smallest. It is known that computing a minmax two-watchman route is NP-hard for simple rectilinear polygons and thus also for simple polygons. Also, any c-approximation algorithm for the minmax two-watchman route is automatically a 2c-approximation algorithm for the minsum two-watchman route. We exhibit two constant factor approximation algorithms for computing minmax two-watchman routes in simple polygons with approximation factors 5.969 and 11.939, having running times O(n^8) and O(n^4) respectively, where n is the number of vertices of the polygon. We also use the same techniques to obtain a 6.922-approximation for the fixed two-watchman route problem running in O(n^2) time, i.e., when two starting points of the two tours are given as input.

==> math.tex <==
\makeatletter 

\newcommand{\remove}[1]{\relax}

\def\comment#1{{\marginpar[\hfill$\longrightarrow${\color{red}\sf\small#1}]{$\longleftarrow${\color{red}\sf\small#1}}}}

\newcommand{\defeq}{\stackrel{\text{def}}{=}}

\newcommand{\diddy}{\fontsize{4}{6}\selectfont}

%%%% Distances
\newcommand{\len}[1]{\mmath{\|#1\|}}
\newcommand{\maxlen}[1]{\mmath{\len{#1}_{\mbox{\tiny\sf max}}}}
\newcommand{\sumlen}[1]{\mmath{\len{#1}_{\mbox{\tiny\sf sum}}}}

%%%% Planes

\newcommand{\lhp}[1]{\mmath{\Area{L}(#1)}}
\newcommand{\lhpb}[1]{\mmath{\Area{L}\big(#1\big)}}
\newcommand{\rhp}[1]{\mmath{\Area{R}(#1)}}
\newcommand{\rhpb}[1]{\mmath{\Area{R}\big(#1\big)}}
%\newcommand{\lhp}[1]{\mmath{\Area{h}^{\!-}(#1)}}
%\newcommand{\rhp}[1]{\mmath{\Area{h}^{\!+}(#1)}}

%%%% Correspondences

\newcommand{\cut}[1]{\mmath{\Line{c}(#1)}}
\newcommand{\cutb}[1]{\mmath{\Line{c}\big(#1\big)}}
\newcommand{\tour}[1]{\mmath{\Path{t}(#1)}}
\newcommand{\tourb}[1]{\mmath{\Path{t}\big(#1\big)}}

%%%% Symbols
\newcommand{\PP}{\Set{P}}
\newcommand{\GG}{\Set{G}}

\newcommand{\XX}{\Set{X}}
\newcommand{\X}{\Curve{X}}
\newcommand{\Xa}{\mmath{\X_1}}
\newcommand{\Xb}{\mmath{\X_2}}
\renewcommand{\Xi}{\mmath{\X_i}}
%\newcommand{\Xj}{\mmath{\X_j}}
%\newcommand{\Xja}{\mmath{\X_{j,1}}}
%\newcommand{\Xjb}{\mmath{\X_{j,2}}}

\newcommand{\UU}{\Set{U}}
\newcommand{\U}{\Curve{U}}
\newcommand{\Ua}{\mmath{\U_1}}
\newcommand{\Ub}{\mmath{\U_2}}
\newcommand{\Upa}{\mmath{\U'_1}}
\newcommand{\Upb}{\mmath{\U'_2}}
%\newcommand{\Ui}{\mmath{\U_i}}
%\newcommand{\Upa}{\mmath{\U'_1}}
%\newcommand{\Uppa}{\mmath{\U''_1}}
\newcommand{\Uua}{\mmath{\UU_{\u_1}}}
\newcommand{\Uub}{\mmath{\UU_{\u_2}}}

\newcommand{\TT}{\Set{T}}
\newcommand{\T}{\Curve{T}}
\newcommand{\Ta}{\mmath{\T_1}}
\newcommand{\Tb}{\mmath{\T_2}}
\newcommand{\Ti}{\mmath{\T_i}}
\newcommand{\Tbi}{\mmath{\Tb^{(i)}}}

\renewcommand{\SS}{\Set{S}}
\renewcommand{\S}{\Curve{S}}
\newcommand{\Sa}{\mmath{\S_1}}
\newcommand{\Sb}{\mmath{\S_2}}

\newcommand{\Ws}{\mmath{\Curve{W}_{\mbox{\tiny\sf\!opt}}}}
\newcommand{\Wbnd}{\mmath{\Curve{W}_{\mbox{\tiny\sf\!bnd}}}}
\newcommand{\WWt}{\mmath{\Set{W}_{\mbox{\tiny\sf T}}}}
\newcommand{\WWSt}{\mmath{\Set{W}^{*}_{\mbox{\tiny\sf T}}}}
\newcommand{\Wa}{\mmath{\Curve{W}_{1}}}
\newcommand{\Wb}{\mmath{\Curve{W}_{2}}}
\newcommand{\Wc}{\mmathp{\Curve{W}_{\mbox{\tiny\sf C}}}}
\newcommand{\Wpa}{\mmath{\Curve{W}'_{1}}}

\newcommand{\lx}{\mmathp{\Line{l}}}

\newcommand{\BB}{{\mmath{\Set{B}}}}
\newcommand{\BBa}{\mmath{\BB_1}}
\newcommand{\BBb}{\mmath{\BB_2}}
\newcommand{\BBc}{\mmath{\BB_3}}
\newcommand{\BBpa}{\mmath{\BB'_1}}
\newcommand{\BBpb}{\mmath{\BB'_2}}

\newcommand{\CC}{\mmath{\Set{C}}}
\newcommand{\CCa}{\mmath{\CC_1}}
\newcommand{\CCb}{\mmath{\CC_2}}

%\newcommand{\BS}{\mmathp{\Set{B}}}
%\newcommand{\BSa}{\mmath{\Set{B}_1}}
%\newcommand{\BSb}{\mmath{\Set{B}_2}}
%\newcommand{\BSi}{\mmath{\Set{B}_i}}

%\newcommand{\CC}{\mmath{\Area{C}}}
%\newcommand{\Ca}{\mmath{\Area{C}_1}}
%\newcommand{\Cb}{\mmath{\Area{C}_2}}
%\newcommand{\Ci}{\mmath{\Area{C}_i}}
%\newcommand{\Cj}{\mmath{\Area{C}_j}}
%\newcommand{\Ctj}{\mmath{\Area{C}_{3-j}}}

%\newcommand{\C}{\mmathp{\Curve{C}}}
\newcommand{\CS}{\mmathp{\Set{C}}}
%\newcommand{\CSa}{\mmath{\Set{C}_1}}
%\newcommand{\CSb}{\mmath{\Set{C}_2}}
%\newcommand{\CSi}{\mmath{\Set{C}_i}}

\newcommand{\DS}{\mmathp{\Set{D}}}
\newcommand{\Da}{\mmath{\Area{D}_{1}}}
\newcommand{\Dal}{\mmath{\Area{D}^{\tiny\sf L}_{1}}}
\newcommand{\Dar}{\mmath{\Area{D}^{\tiny\sf R}_{1}}}
\newcommand{\Dac}{\mmath{\Area{D}^{\tiny\sf C}_{1}}}
\newcommand{\Dax}{\mmath{\Area{D}^{\tiny\sf X}_{1}}}

%\newcommand{\Pb}{\mmathp{\Curve{P}_2}}
%\newcommand{\Pc}{\mmathp{\Curve{P}_3}}
%\newcommand{\Pd}{\mmathp{\Curve{P}_4}}
%\newcommand{\Pj}{\mmathp{\Curve{P}_j}}
%\newcommand{\Pm}{\mmathp{\Curve{P}_m}}

\newcommand{\PS}{\mmathp{\Set{P}}}

%\newcommand{\shp}{\mmathp{\Curve{P}}}

\newcommand{\VV}{\mmath{\Set{V}}}
\newcommand{\Va}{\mmathp{\Curve{V}_1}}
\newcommand{\Vb}{\mmathp{\Curve{V}_2}}
\newcommand{\V}{\mmathp{\Curve{V}}}
\newcommand{\Vj}{\mmathp{\Curve{V}_j}}
\newcommand{\Vi}{\mmathp{\Curve{V}_i}}

\newcommand{\EE}{\mmath{\Set{E}}}
\newcommand{\Ea}{\mmath{\Set{E}_1}}
\newcommand{\Eb}{\mmath{\Set{E}_2}}
\newcommand{\Ei}{\mmath{\Set{E}_i}}

\newcommand{\ex}{\mmathp{\Line{e}}}

\newcommand{\e}{\mmathp{\Line{e}}}
\newcommand{\ei}{\mmathp{\e_i}}
\newcommand{\et}{\mmathp{\e_{3-i}}}
\newcommand{\ej}{\mmathp{\e_j}}
\newcommand{\eA}{\mmathp{\e_{\!\Polygon{A}}}}
\newcommand{\eB}{\mmathp{\e_{\Polygon{B}}}}
\newcommand{\eia}{\mmathp{\e^{\mbox{\diddy$(i)$}}_1}}
\newcommand{\eib}{\mmathp{\e^{\mbox{\diddy$(i)$}}_2}}
\newcommand{\eij}{\mmathp{\e^{\mbox{\diddy$(i)$}}_j}}
\newcommand{\eijp}{\mmathp{\e^{\mbox{\diddy$(i)$}}_{j+1}}}
\newcommand{\eimi}{\mmathp{\e^{\mbox{\diddy$(i)$}}_{\raisebox{0ex}[1ex]{\scriptsize\mi}}}}

\newcommand{\mi}{\mmath{m^{\mbox{\diddy$(i)$}}}}

\newcommand{\ls}{\mmath{\Line{l}}}
\newcommand{\lss}{\mmath{\Line{l}^{*}}}

\newcommand{\be}{\mmathp{\Line{b}}}
\newcommand{\bea}{\mmathp{\Line{b}_1}}
\newcommand{\beb}{\mmathp{\Line{b}_2}}
\newcommand{\bee}{\mmath{\Line{b}_{\e}}}
\newcommand{\bei}{\mmathp{\Line{b}_i}}
\newcommand{\bej}{\mmathp{\Line{b}_j}}

\newcommand{\ssa}{\mmathp{\Line{s}_{1}}}
\newcommand{\ssb}{\mmathp{\Line{s}_{2}}}
%\newcommand{\se}{\mmath{\Line{s_{\e}}}}
\newcommand{\sei}{\mmath{\Line{s_{\ei}}}}
\newcommand{\sbe}{\mmathp{\Line{s}_{\be}}}
%\newcommand{\sbei}{\mmath{\Line{s}_{\be_i}}}
%\newcommand{\sbea}{\mmath{\Line{s}_{\be_1}}}
%\newcommand{\sbeb}{\mmath{\Line{s}_{\be_2}}}

\newcommand{\uh}{\mmathp{u_{h}}}
%\newcommand{\uep}{\mmath{u_{\e'}}}
%\newcommand{\uei}{\mmath{u_{\ei}}}
%\newcommand{\ueir}{\mmath{u_{\eir}}}

\newcommand{\ea}{\mmath{\Line{e}_1}}
\newcommand{\eb}{\mmath{\Line{e}_2}}
%\newcommand{\ec}{\mmath{\Line{e}_3}}

\newcommand{\p}{\mmathp{\Point{p}}}
\newcommand{\pa}{\mmathp{\Point{p}_1}}
\newcommand{\pb}{\mmathp{\Point{p}_2}}
\newcommand{\pc}{\mmathp{\Point{p}_3}}
\newcommand{\pj}{\mmathp{\Point{p}_j}}
\newcommand{\paL}{\mmath{\Point{p}_{\mbox{\tiny\sf L}}}}
\newcommand{\paR}{\mmath{\Point{p}_{\mbox{\tiny\sf R}}}}
%\newcommand{\pii}{\mmathp{\Point{p}^{(i)}}}
\newcommand{\pia}{\mmathp{\Point{p}^{\mbox{\diddy$(i)$}}_1}}
\newcommand{\pib}{\mmathp{\Point{p}^{\mbox{\diddy$(i)$}}_2}}
%\newcommand{\pij}{\mmathp{\Point{p}^{(i)}_{j}}}


\newcommand{\pt}{\mmathp{\tilde{\Point{p}}}}
\newcommand{\ptx}{\mmathp{\tilde{\Point{p}}_x}}
\newcommand{\pty}{\mmathp{\tilde{\Point{p}}_y}}
\newcommand{\ph}{\mmathp{\bar{\Point{p}}}}

\newcommand{\px}{\mmath{\p_x}}



\newcommand{\aia}{\mmath{\alpha^{\mbox{\diddy$(i)$}}_{1}}}



\newcommand{\q}{\mmathp{\Point{q}}}
\newcommand{\qa}{\mmath{\Point{q}_1}}
\newcommand{\qb}{\mmath{\Point{q}_2}}
\newcommand{\qi}{\mmathp{\Point{q}_i}}
\newcommand{\qsa}{\mmath{\Point{q}^{*}_1}}
\newcommand{\qsb}{\mmath{\Point{q}^{*}_2}}
\newcommand{\qss}{\mmath{\Point{q}^{*}}}
\newcommand{\qs}{\mmathp{\Point{q}_{*}^{}}}
\newcommand{\qsp}{\mmathp{\Point{q}_{*}^{\prime}}}
%\newcommand{\qij}{\mmathp{\Point{q}_{ij}}}
\newcommand{\qija}{\mmathp{\Point{q}_{\e_1}}}
\newcommand{\qijb}{\mmathp{\Point{q}_{\e_2}}}

\newcommand{\qaa}{\mmath{\Point{q}^{\mbox{\diddy(1)}}_1}}
\newcommand{\qab}{\mmath{\Point{q}^{\mbox{\diddy(1)}}_2}}
\newcommand{\qba}{\mmath{\Point{q}^{\mbox{\diddy(2)}}_1}}
\newcommand{\qbb}{\mmath{\Point{q}^{\mbox{\diddy(2)}}_2}}
\newcommand{\qca}{\mmath{\Point{q}^{\mbox{\diddy(3)}}_1}}
\newcommand{\qcb}{\mmath{\Point{q}^{\mbox{\diddy(3)}}_2}}
\newcommand{\qda}{\mmath{\Point{q}^{\mbox{\diddy(4)}}_1}}
\newcommand{\qdb}{\mmath{\Point{q}^{\mbox{\diddy(4)}}_2}}
\newcommand{\qea}{\mmath{\Point{q}^{\mbox{\diddy(5)}}_1}}
\newcommand{\qeb}{\mmath{\Point{q}^{\mbox{\diddy(5)}}_2}}

\newcommand{\qiia}{\mmathp{\Point{q}_{\e_{1}}}}
\newcommand{\qiib}{\mmathp{\Point{q}_{\e_{2}}}}
\newcommand{\qei}{\mmathp{\Point{q}_{\e_{i}}}}
\newcommand{\qet}{\mmathp{\Point{q}_{\e_{3-i}}}}
\newcommand{\qh}{\mmathp{\hat{\Point{q}}}}

%\renewcommand{\r}{\mmathp{\Point{r}}}
\newcommand{\rr}{\mmathp{\Point{r}}}
\newcommand{\ra}{\mmath{\Point{r}_1}}
\newcommand{\rb}{\mmath{\Point{r}_2}}
\newcommand{\rs}{\mmath{\Point{r}^{*}}}
\newcommand{\rsa}{\mmath{\Point{r}^{*}_1}}
\newcommand{\rsb}{\mmath{\Point{r}^{*}_2}}
\newcommand{\rc}{\mmath{\Point{r}^{\dag}}}
%\newcommand{\rsa}{\mmath{\Point{r}^{*}_1}}
%\newcommand{\rsb}{\mmath{\Point{r}^{*}_2}}
\newcommand{\ri}{\mmath{\Point{r}_i}}
\newcommand{\rj}{\mmath{\Point{r}_j}}
\newcommand{\rip}{\mmath{\Point{r}'_i}}
\newcommand{\rjp}{\mmath{\Point{r}'_j}}
%\newcommand{\rij}{\mmath{\Point{r}_{ij}}}
%\newcommand{\ria}{\mmath{\Point{r}_{i,1}}}
%\newcommand{\rib}{\mmath{\Point{r}_{i,2}}}
\newcommand{\rx}{\mmathp{\rr_x}}
\newcommand{\ry}{\mmathp{\rr_y}}


%\newcommand{\riaj}{\mmath{\Point{r}^{(i)}_{1,j}}}
%\newcommand{\ribj}{\mmath{\Point{r}^{(i)}_{2,j}}}
\newcommand{\riaa}{\mmath{\Point{r}^{\mbox{\diddy$(i)$}}_{1,1}}}
\newcommand{\riba}{\mmath{\Point{r}^{\mbox{\diddy$(i)$}}_{2,1}}}
\newcommand{\riab}{\mmath{\Point{r}^{\mbox{\diddy$(i)$}}_{1,2}}}
\newcommand{\rias}{\mmath{\Point{r}^{\mbox{\diddy$(i)$}}_{1,*}}}
\newcommand{\ribs}{\mmath{\Point{r}^{\mbox{\diddy$(i)$}}_{2,*}}}
%\newcommand{\rimip}{\mmath{\Point{r}^{(i)}_{\mi+1}}}


\newcommand{\ta}{\mmath{\Point{t}_1}}
\newcommand{\tb}{\mmath{\Point{t}_2}}

\newcommand{\w}{\mmathp{\Line{w}}}
%\newcommand{\wL}{\mmath{\w_{l}}}
%\newcommand{\wR}{\mmath{\w_{r}}}
\newcommand{\wa}{\mmath{\Line{w}_{1}}}
\newcommand{\wb}{\mmath{\Line{w}_{2}}}

\renewcommand{\v}{\mmathp{\Point{v}}}
\renewcommand{\u}{\mmathp{\Point{u}}}
\newcommand{\vi}{\mmathp{\Point{v}^{}_i}}
\newcommand{\vii}{\mmathp{\Point{v}_i}}
\newcommand{\vip}{\mmath{\Point{v}'_i}}
\newcommand{\vj}{\mmathp{\Point{v}^{}_j}}
\newcommand{\vjp}{\mmath{\Point{v}'_j}}
\newcommand{\via}{\mmath{\Point{v}^{\mbox{\diddy$(i)$}}_{1}}}
\newcommand{\vib}{\mmath{\Point{v}^{\mbox{\diddy$(i)$}}_2}}
%\newcommand{\vij}{\mmath{\Point{v}^{(i)}_j}}
%\newcommand{\vijp}{\mmath{\Point{v}^{(i)}_{j+1}}}
\newcommand{\vimi}{\mmath{\Point{v}^{\mbox{\diddy$(i)$}}_{\raisebox{0ex}[1ex]{\scriptsize\mi}}}}

\newcommand{\vx}{\mmathp{\v_x}}
\newcommand{\vy}{\mmathp{\v_y}}
\newcommand{\ux}{\mmathp{\u_x}}
\newcommand{\uy}{\mmathp{\u_y}}

\newcommand{\va}{\mmath{\Point{v}_1^{}}}
\newcommand{\vb}{\mmath{\Point{v}_2^{}}}
\newcommand{\vap}{\mmath{\Point{v}_1^{\prime}}}
\newcommand{\vbp}{\mmath{\Point{v}_2^{\prime}}}
%\newcommand{\ve}{\mmath{\Point{v}_{\e}}}

\newcommand{\ua}{\mmathp{\Point{u}_1}}
\newcommand{\ub}{\mmathp{\Point{u}_2}}
\newcommand{\uc}{\mmathp{\Point{u}_3}}
\newcommand{\ui}{\mmathp{\Point{u}_i}}
\newcommand{\uia}{\mmath{\Point{u}^{\mbox{\diddy$(i)$}}_1}}
\newcommand{\uib}{\mmath{\Point{u}^{\mbox{\diddy$(i)$}}_2}}
\newcommand{\uaa}{\mmath{\Point{u}^{\mbox{\diddy$(1)$}}_1}}
\newcommand{\ukb}{\mmath{\Point{u}^{\mbox{\diddy$(k)$}}_2}}
\newcommand{\uimi}{\mmath{\Point{u}^{\mbox{\diddy$(i)$}}_{\raisebox{0ex}[1ex]{\scriptsize\mi}}}}

\newcommand{\C}{\mmathp{\Curve{C}}}
\newcommand{\Ci}{\mmath{\Curve{C}^{\mbox{\diddy$(i)$}}}}
\newcommand{\Cbi}{\mmath{\Curve{\bar{C}}^{\mbox{\diddy$(i)$}}}}
\newcommand{\Cbiam}{\mmath{\Curve{\bar{C}}^{\mbox{\diddy$(i)$}}\!\big({\uia,\uimi}\big)}}
\newcommand{\Cbiab}{\mmath{\Curve{\bar{C}}^{\mbox{\diddy$(i)$}}\!\big({\uia,\vib}\big)}}
\newcommand{\Cbibm}{\mmath{\Curve{\bar{C}}^{\mbox{\diddy$(i)$}}\!\big({\vib,\uimi}\big)}}
%\newcommand{\Cpi}{\mmath{{\Curve{\bar{C}}}^{(i)}}}
\newcommand{\Ca}{\mmath{\Curve{C}_1}}
\newcommand{\Cb}{\mmath{\Curve{C}_2}}
%\newcommand{\Ck}{\mmath{\Curve{C}_k}}


\newcommand{\s}{\mmathp{\Line{s}}}
%\renewcommand{\t}{\mmathp{\Line{t}}}

%\let\new@Pi=\Pi
%\renewcommand{\Pi}{\mmath{\new@Pi}}
\renewcommand{\P}{\Polygon{P}}
\newcommand{\PL}{\mmath{\P_{\!L}}}
\newcommand{\PR}{\mmath{\P_{\!R}}}
\newcommand{\Pxa}{\mmath{\Polygon{P}_{\!\Xa}}}
\newcommand{\Pxb}{\mmath{\Polygon{P}_{\!\Xb}}}
%\newcommand{\Pva}{\mmath{\Polygon{P}_{\!\Va}}}
%\newcommand{\Pvb}{\mmath{\Polygon{P}_{\!\Vb}}}
\newcommand{\Pp}{\mmath{\Polygon{P}_{\!\p}}}

\newcommand{\Pz}{\mmathp{\P_{\!0}}}
\newcommand{\Pa}{\mmathp{\P_{\!1}}}

\newcommand{\Pex}{\mmath{\P_{\!\!\ex}}}
%\newcommand{\Pcx}{\mmath{\bar{\P}_{\!\!\ex}}}
\newcommand{\Peu}{\mmath{\P_{\!\!\ex(\u)}}}
\newcommand{\Peup}{\mmath{\P_{\!\!\ex(\u')}}}
\newcommand{\Plu}{\mmath{\P_{\!\lx(\u)}}}
%\newcommand{\Pev}{\mmath{\P_{\!\!\ex(\v)}}}
\newcommand{\Pe}{\mmathp{\P_{\!\e}}}
\newcommand{\Pne}{\mmath{\bar{\P}_{\!\e}}}
\newcommand{\Pc}{\mmathp{\P_{\!\Polygon{c}}}}

\newcommand{\dP}{\mmath{\partial\P}}
\newcommand{\dPa}{\mmath{\partial\P_{\!1}}}
\newcommand{\dPb}{\mmath{\partial\P_{\!2}}}
\newcommand{\OPT}{\mmath{{\it OPT}}}
%\newcommand{\LL}[1]{\mmath{\Polygon{L}_{#1}}}
\newcommand{\RR}{\mmath{\Polygon{R}}}
\newcommand{\Rp}{\mmath{\RR'}}
\newcommand{\Ri}{\mmath{\RR_i}}
\newcommand{\Rip}{\mmath{\RR'_i}}
\newcommand{\QQ}{\mmathp{\Polygon{Q}}}


\newcommand{\LL}{\mmathp{\Set{L}}}


\newcommand{\VP}[1]{{\mmath{\Polygon{VP}(#1)}}}

\newcommand{\Dij}[1]{\mmath{\Function{D}_{ij}(#1)}}
\newcommand{\Dii}[1]{\mmath{\Function{D}_{ii}(#1)}}
\newcommand{\Djj}[1]{\mmath{\Function{D}_{jj}(#1)}}
\newcommand{\DD}[1]{\mmath{\Function{D}(#1)}}
\newcommand{\Fa}{\mmath{\Set{F}_{1}}}
\newcommand{\Fb}{\mmath{\Set{F}_{2}}}
\newcommand{\Fi}{\mmath{\Set{F}_{i}}}
\newcommand{\Fpa}{\mmath{\Set{F}'_{1}}}
\newcommand{\Fai}{\mmath{\Fa^{(i)}}}

\newcommand{\Pil}{{\mmath{\Pi_{L}}}}
\newcommand{\Pir}{{\mmath{\Pi_{R}}}}
\newcommand{\Pim}{{\mmath{\Pi_{M}}}}


\newcommand{\dd}{\mmathp{d}}

\newcommand{\vbar}{\mmathp{\bar{\Point{v}}}}


\newcommand{\JJ}{\mmathp{\Set{J}}}

\def\SP(#1){\mmath{\Curve{SP}(#1)}}
\def\SPb(#1){\mmath{\Curve{SP}\big(#1\big)}}
\def\SPR(#1){\mmath{\Curve{SP}_{\!R}(#1)}}
\def\JF(#1,#2){\mmath{\Set{J}_{#1,#2}}}
\def\JFs(#1){\mmath{\Set{J}_{#1}}}
\def\ZT(#1,#2){\mmath{\Curve{Z}_{#1}^{#2}}}
\def\ZR(#1,#2,#3){\mmath{\Curve{Z}_{#1}^{#2}\!(#3)}}
\def\MJF(#1,#2){{\mmath{\Set{J}^{\min}_{#1,#2}}}}
\def\MJFs(#1){\mmath{\Set{J}^{\min}_{#1}}}
\def\MJR(#1,#2){{\mmath{\Set{J}^{\rm red}_{#1,#2}}}}
\def\MJRs(#1){\mmath{\Set{J}^{\rm red}_{#1}}}
\def\MJWs(#1){\mmath{\Set{J}^{\mbox{\tiny\sf2}}_{#1}}}


\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\makeatother
